Self-labelling via simultaneous clustering and representation learning

Combining clustering and representation learning is one of the most promising approaches for unsupervised learning of deep neural networks. However, doing so naively leads to ill posed learning problems with degenerate solutions. In this paper, we propose a novel and principled learning formulation that addresses these issues. The method is obtained by maximizing the information between labels and input data indices. We show that this criterion extends standard crossentropy minimization to an optimal transport problem, which we solve efficiently for millions of input images and thousands of labels using a fast variant of the Sinkhorn-Knopp algorithm. The resulting method is able to self-label visual data so as to train highly competitive image representations without manual labels. Our method achieves state of the art representation learning performance for AlexNet and ResNet-50 on SVHN, CIFAR-10, CIFAR-100 and ImageNet and yields the first self-supervised AlexNet that outperforms the supervised Pascal VOC detection baseline. Code and models are available.

==> figs/fig-method.tex <==
\begin{figure}[!tb]
\centering
\includegraphics[width=0.95\linewidth]{figs/self-lab-method.pdf}
\caption{\textbf{yuki: Maybe the figure doesn't add much, as our method is quite easy to understand. But that's also our strength so it might be good. } The method proposed in this paper along with the visualization of the first convolutional layer of a trained AlexNet.  \label{fig:method}}
\end{figure}

==> figs/fig1.tex <==
\begin{figure}[!h]
\centering
\includegraphics[width=0.9\linewidth]{figs/fig1draft.png}
\caption{Out method gives visually similar clusters without using labels...\label{fig:method}
\todo{add space between top,middle,bottom and add three dots. add entropy axis}}
\end{figure}


==> figs/fig2.tex <==
\begin{figure}[!tb]
\centering
\includegraphics[width=0.5\linewidth]{figs/fig2draft.png}
\caption{\textbf{yuki: maybe we don't need this figure. It doesn't tell us much. }Top: entropy of all the pseudolabels with regards to the true imagenet train labels. Bottom: evolution of a good cluster.\label{fig:evolution}
\todo{add time in epochs as colorbar}}
\end{figure}


==> tables/apx-tab-linear.tex <==
\setlength{\tabcolsep}{2pt}
\begin{table}[!h]
  \centering
  \caption{
    \textbf{2012 AlexNet performances.} A linear classifier is trained on the (downsampled) activations of each layer in the pretrained model. See text for technical details. 
  }
    \begin{tabular}{l rrrrr}
      \toprule
            & \multicolumn{5}{c}{ILSVRC-12}\\
      Method   & \texttt{c1} & \texttt{c2} & \texttt{c3} & \texttt{c4} & \texttt{c5} \\
      \midrule
      ImageNet labels (10-crop)$^*$ & $22.7$ & $39.7$ & $52.3$ & $59.6$ & $61.3$\\
      ImageNet labels (1-crop)$^*$ & $20.5$ & $33.9$ & $41.9$ & $47.4$ & $49.2$ \\
      Random (10-crop)$^*$& $17.6$ & $20.3$ & $20.6$ & $17.8$ & $11.0$ \\
      Random (1-crop)$^*$ & $15.6$ & $16.8$ & $17.4$ & $15.6$ & $10.6$ \\
      \bottomrule
    \end{tabular}
  
  \label{tab:app-linear}
\end{table}


==> tables/result_macros.tex <==
\newcommand\res_3x1k{}
